Assessing Test Case Prioritization on Real Faults and Mutants

Test Case Prioritization (TCP) is an important component of regression testing, allowing for earlier detection of faults or helping to reduce testing time and cost. While several TCP approaches exist in the research literature, a growing number of studies have evaluated them against synthetic software defects, called mutants. Hence, it is currently unclear to what extent TCP performance on mutants would be representative of the performance achieved on real faults. To answer this fundamental question, we conduct the first empirical study comparing the performance of TCP techniques applied to both real-world and mutation faults. The context of our study includes eight well-studied TCP approaches, 35k+ mutation faults, and 357 real-world faults from five Java systems in the Defects4J dataset. Our results indicate that the relative performance of the studied TCP techniques on mutants may not strongly correlate with performance on real faults, depending upon attributes of the subject programs. This suggests that, in certain contexts, the best performing technique on a set of mutants may not be the best technique in practice when applied to real faults. We also illustrate that these correlations vary for mutants generated by different operators depending on whether chosen operators reflect typical faults of a subject program. This highlights the importance, particularly for TCP, of developing mutation operators tailored for specific program domains.

==> discussion.tex <==
% !TEX root = main.tex

\section{Dicussion} 

==> macro.tex <==


\usepackage{amssymb}
\usepackage{ifthen}

\makeatletter

% this  is a easy way to add and highlight new text  ...
% just comment in/out the \tnew macro ..

\newcommand{\tnew}[1]{{\bf { #1 }} }
%\newcommand{\tnew}[1]{{ { #1 }} }

% math and theorem definition

\newcommand{\ndef}{\stackrel{\rm def}{=}}

% this is used for draft only

%\renewcommand{\baselinestretch}{2}

% just to number pages in the draft

\pagenumbering{arabic}

% nothing i.e., no-numbering final and camera ready

%\pagestyle{empty}


\newboolean{showcomments}


\setboolean{showcomments}{true}

\ifthenelse{\boolean{showcomments}}
  {\newcommand{\nb}[2]{
    \fbox{\bfseries\sffamily\scriptsize#1}
    {\sf\small$\blacktriangleright$\textit{#2}$\blacktriangleleft$}
   }
   \newcommand{\cvsversion}{\emph{\scriptsize$-$Id: macro.tex,v 1.9 2005/12/09 22:38:33 giulio Exp $}}
  }
  {\newcommand{\nb}[2]{}
   \newcommand{\cvsversion}{}
  }


\newcommand\DENYS[1]{\textcolor{blue}{\nb{DENYS}{#1}}}
\newcommand\QI[1]{\textcolor{blue}{\nb{QI}{#1}}}
\newcommand\KEVIN[1]{\textcolor{blue}{\nb{KEVIN}{#1}}}
\newcommand\MAX[1]{\textcolor{blue}{\nb{MAX}{#1}}}
\newcommand\revision[1]{{#1}}






==> tables/coupling-perf.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table*}[t]
\centering
\footnotesize
\vspace{-0.2cm}
\definecolor{mygray}{gray}{0.9}
\caption{\small APFD values for TCP techniques in terms of detecting different types of real faults. Couple refers to the real faults coupled with mutation faults. StrongerOP refers to the real faults requiring stronger mutation operators. NewOP refers to the real faults requiring new mutation operators. Limitation refers the real faults not coupled with mutation faults.}
\vspace{-0.2cm}
\label{my-label}
\begin{tabular}{|c|c|c!{\vrule width 0.8pt}c|c!{\vrule width 0.8pt}c|c!{\vrule width 0.8pt}c|c!{\vrule width 0.8pt}c|c!{\vrule width 0.8pt}c|c!{\vrule width 0.8pt}c|c!{\vrule width 0.8pt}c|c!{\vrule width 0.8pt}}
\hline
Real Faults & \multicolumn{2}{c!{\vrule width 0.8pt}}{TCP$_{cg-tot}$}        & \multicolumn{2}{c!{\vrule width 0.8pt}}{TCP$_{cg-add}$}        & \multicolumn{2}{c!{\vrule width 0.8pt}}{TCP$_{str}$}           & \multicolumn{2}{c!{\vrule width 0.8pt}}{TCP$_{topic}$}         & \multicolumn{2}{c!{\vrule width 0.8pt}}{TCP$_{total}$}         & \multicolumn{2}{c!{\vrule width 0.8pt}}{TCP$_{add}$}           & \multicolumn{2}{c!{\vrule width 0.8pt}}{TCP$_{art}$}           & \multicolumn{2}{c!{\vrule width 0.8pt}}{TCP$_{search}$}        \\ \hline\hline
            & APFD  & {\cellcolor{mygray}}APFDc & APFD  & {\cellcolor{mygray}}APFDc & APFD  & {\cellcolor{mygray}}APFDc & APFD  & {\cellcolor{mygray}}APFDc & APFD  & {\cellcolor{mygray}}APFDc & APFD  & {\cellcolor{mygray}}APFDc & APFD  & {\cellcolor{mygray}}APFDc & APFD  & {\cellcolor{mygray}}APFDc \\ \hlinewd{0.7pt}
Couple      & 0.577 & {\cellcolor{mygray}}0.479 & 0.581 & {\cellcolor{mygray}}0.583 & 0.689 & {\cellcolor{mygray}}0.594 & 0.688 & {\cellcolor{mygray}}0.631 & 0.625 & {\cellcolor{mygray}}0.439 & 0.589 & {\cellcolor{mygray}}0.462 & 0.642 & {\cellcolor{mygray}}0.675 & 0.597 & {\cellcolor{mygray}}0.56  \\ \hline
Limitation  & 0.669 & {\cellcolor{mygray}}0.491 & 0.617 & {\cellcolor{mygray}}0.608 & 0.696 & {\cellcolor{mygray}}0.56  & 0.695 & {\cellcolor{mygray}}0.605 & 0.571 & {\cellcolor{mygray}}0.387 & 0.552 & {\cellcolor{mygray}}0.422 & 0.748 & {\cellcolor{mygray}}0.717 & 0.637 & {\cellcolor{mygray}}0.578 \\ \hline
StrongerOP  & 0.695 & {\cellcolor{mygray}}0.564 & 0.652 & {\cellcolor{mygray}}0.649 & 0.767 & {\cellcolor{mygray}}0.676 & 0.756 & {\cellcolor{mygray}}0.703 & 0.488 & {\cellcolor{mygray}}0.267 & 0.575 & {\cellcolor{mygray}}0.476 & 0.698 & {\cellcolor{mygray}}0.702 & 0.619 & {\cellcolor{mygray}}0.572 \\ \hline
NewOP       & 0.333 & {\cellcolor{mygray}}0.16  & 0.706 & {\cellcolor{mygray}}0.692 & 0.639 & {\cellcolor{mygray}}0.595 & 0.662 & {\cellcolor{mygray}}0.604 & 0.191 & {\cellcolor{mygray}}0.081 & 0.512 & {\cellcolor{mygray}}0.377 & 0.707 & {\cellcolor{mygray}}0.796 & 0.549 & {\cellcolor{mygray}}0.506 \\ \hline
\end{tabular}
\end{table*}

==> tables/static-dynamic.tex <==

\begin{table}[t]
\small
\centering
\vspace{-0.2cm}
\definecolor{mygray}{gray}{0.9}
\revision{
\caption{\small Results of Wilcoxon Rank Sum Test for Static Techniques Compared to Dynamic Techniques, with p-values and effect size}
\label{tab:static-dynamic}
\vspace{-0.25cm}
\begin{tabular}{|c!{\vrule width 0.8pt}c|c!{\vrule width 0.8pt}c|c|c|}
\hline
Faults                 & \multicolumn{2}{c!{\vrule width 0.8pt}}{Wilcoxon $p$-value} & \multicolumn{2}{c|}{Cliff's $\delta$} & Effect Size                         \\ \hline\hline
\multicolumn{1}{|l!{\vrule width 0.8pt}}{} & APFD          & {\cellcolor{mygray}}APFDc        & APFD                   & {\cellcolor{mygray}}APFDc  &    APFD(c)            \\ \hlinewd{0.7pt}
Real            & 0.142        & {\cellcolor{mygray}}0.314      &  0.275 & \cellcolor{mygray} {0.190} & small \\ 
Mutant           & 0.738          & {\cellcolor{mygray}}0.820      & 0.065 & \cellcolor{mygray}{0.045} & negligable\\ 
S.Mutant           & 0.718     & {\cellcolor{mygray}}0.511      &  0.070  &    \cellcolor{mygray}0.125 &  negligable          \\\arrayrulecolor{black}\hline
\end{tabular}
\vspace{-0.65cm}}
\end{table}

==> tables/subMut.tex <==
\begin{table*}[t]
\center
%\vspace{-0.5cm}
%\scriptsize
%\tiny
\footnotesize
\caption{APFD values for TCP techniques in terms of detecting different types of mutation faults. The mutation faults are classified based on their corresponding mutation operators. \label{table:subMut}\vspace{-0.2cm}}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
\hline
Mutation Faults&{TCP$_{cg-tot}$}&{TCP$_{cg-add}$}&{TCP$_{str}$}&{TCP$_{topic}$}&{TCP$_{total}$}&{TCP$_{add}$}&{TCP$_{art}$}&{TCP$_{search}$}\\
\hline\hline
NegateConditionals&0.751&0.838&0.854&0.853&0.775&0.916&0.823&0.806\\\hline
RemoveConditional&0.759&0.842&0.858&0.857&0.782&0.921&0.83&0.814\\\hline
ConstructorCall&0.749&0.801&0.815&0.818&0.739&0.882&0.799&0.773\\\hline
NonVoidMethodCall&0.755&0.815&0.823&0.823&0.76&0.889&0.783&0.78\\\hline
Math&0.713&0.758&0.815&0.798&0.692&0.887&0.797&0.765\\\hline
MemberVariable&0.752&0.845&0.835&0.827&0.776&0.904&0.824&0.789\\\hline
InlineConstant&0.711&0.784&0.836&0.824&0.721&0.887&0.794&0.757\\\hline
Increments&0.779&0.833&0.861&0.858&0.767&0.94&0.844&0.826\\\hline
ArgumentPropagation&0.751&0.799&0.829&0.814&0.749&0.875&0.767&0.775\\\hline
ConditionalsBoundary&0.751&0.788&0.846&0.837&0.734&0.907&0.806&0.784\\\hline
Switch&0.833&0.925&0.917&0.939&0.891&0.969&0.865&0.887\\\hline
VoidMethodCall&0.735&0.791&0.763&0.78&0.764&0.868&0.721&0.76\\\hline
InvertNegs&0.781&0.784&0.888&0.856&0.753&0.927&0.818&0.803\\\hline
ReturnVals&0.71&0.82&0.814&0.813&0.711&0.87&0.796&0.758\\\hline
RemoveIncrements&0.769&0.813&0.865&0.856&0.774&0.924&0.826&0.811\\\hline
\end{tabular}
\vspace{-0.3cm}
\end{table*}

